A General Method for Deriving Tight Symbolic Bounds on Causal Effects

A causal query will commonly not be identifiable from observed data, in which case no estimator of the query can be contrived without further assumptions or measured variables, regardless of the amount or precision of the measurements of observed variables. However, it may still be possible to derive symbolic bounds on the query in terms of the distribution of observed variables. Bounds, numeric or symbolic, can often be more valuable than a statistical estimator derived under implausible assumptions. Symbolic bounds, however, provide a measure of uncertainty and information loss due to the lack of an identifiable estimand even in the absence of data. We develop and describe a general approach for computation of symbolic bounds and characterize a class of settings in which our method is guaranteed to provide tight valid bounds. This expands the known settings in which tight causal bounds are solutions to linear programs. We also prove that our method can provide valid and possibly informative symbolic bounds that are not guaranteed to be tight in a larger class of problems. We illustrate the use and interpretation of our algorithms in three examples in which we derive novel symbolic bounds.

==> depsup.tex <==

\section{On the informativeness of the bounds}


DAGs that include unmeasured outcome variables are within this class of problems. However, not all cases will provide useful bounds, meaning bounds that are more narrow than the maximum and minimum possible values of the target parameter without any information. For example, for the risk difference from -1 to 1. Although there are many possible problems within our class which will result in useless bounds, we outline two cases where this will always be the case, so that they can be avoided. 

One example is a setting where all outcomes within the target are unobserved and there are either no children of any of these outcomes or they are all also unobserved. Of course in this setting you could set constants that provide informative bounds, but that would occur even in the absence of any information. 


\begin{theorem}
Beyond those implied by the assumed constraints, the tight bounds will not be informative unless there is at least one outcome or child or grandchild etc. of one of the outcomes that is observed. 
\end{theorem}

\subsection*{Proof}

For the bounds on an outcome to be informative the observed data must provide a means of bounding away from zero or 1 at least one of the joint counterfactual probabilities involving the outcome. Without loss of generality assume we have a single unobserved outcome of interest without observed children. Then let the joint probabilities on the counterfactuals be $q_{y,x\ldots b}$.

Let us start by assuming no constraints on the relationships so all $q_{y,x\ldots b}$ are possibly $>0$. Consider $P\{Y(x=1, \ldots b=1)=0\}$ the possible observed probabilities that map to this are $P_{x=1 \ldots b=1}$. However, this is the same exact probability that maps to $P\{Y(x=1, \ldots b=1)=1\}$, therefore regardless of the values of $P_{x=1 \ldots b=1}$ we cannot bound counterfactual probabilities for $Y$ because we cannot differentiate between $P(Y=1)$ and $P(Y=0)$. Therefore, any bounds derived for $P\{Y(x=1, \ldots b=1)=0\}$ would equally apply for $P\{Y(x=1, \ldots b=1)=1\}$. However, this group is also what would apply to the difference or sum of these two values. 

$P\{Y(x=1, \ldots b=1)=0\}-P\{Y(x=1, \ldots b=1)=1\} = \pm P_{x=1 \ldots b=1}$ which could be true if $P\{Y(x=1, \ldots b=1)=0\}=P_{x+1 \ldots b=1}$ or $P\{Y(x=1, \ldots b=1)=1\}=P_{x=1 \ldots b=1}$, but we cannot differentiate between these. Therefore, $P\{Y(x=1, \ldots b=1)=0\}$ is only bounded between 0 and $P_{x=1 \ldots b=1}$, as is $P\{Y(x=1, \ldots b=1)=1\}$ making the only narrowing of the interval from -1 to 1, the information contained in $P_{x=1 \ldots b=1}$. Without any constraints on the $q$s,  $P_{x=1 \ldots b=1}$, can be 0 and 1. This can be similarly be applied to any set of the $x \ldots b$, and thus there exist no $P\{Y(x, \ldots b)=0\}$ or $P\{Y(x, \ldots b)=1\}$ that can be bounded. 


==> latexmkrc <==
# HACK: this width seems to change with every compile, so
# latexmk runs latex too many times; ignore it
$hash_calc_ignore_pattern{'aux'} = 'statsocwidth';

# All the other default settings on Overleaf
# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}
